Bounds for inertialess dynamo

We derive necessary conditions for instantaneous dynamo action for rotating convection. A magnetohydrodynamic model is considered in two settings: the rapidly rotating plane layer where inertia and viscosity are absent, and at an arbitrary rotation rate where viscosity is finite. In contrast to kinematic dynamo bounds, the evolution of the magnetic field is coupled via an inertialess force balance. The buoyancy-driven part of the flow $\mathbf{u}^{\mathrm{A}}$ in the event of dynamo action must in fact satisfy, for $3\leq p \leq \infty$ $$ Rm\, A_p\| \mathbf{u}^{\mathrm{A}}\|_{L^p} \geq 1 $$ where $A_p$ is an explicit constant, and $Rm$ is the magnetic Reynolds number. In the inviscid model, $\mathbf{u}^{\mathrm{A}}$ depends only on the horizontal gradients of the vertical primitive of temperature. A refinement via the poloidal-toroidal decomposition allows us to replace $L^p$ in our constraint with an anisotropic norm for $L^{\infty}_z \dot{H}^1_{x,y}$. For the viscous model, we also derive necessary conditions for the growth of magnetic enstrophy and a combined thermo-magnetic energy. One branch of our constraints implies that the scaling $Ra_\nu \gtrsim Ek^{-3/2}$ is necessary for dynamo action, where $Ra_\nu$ is the classical Rayleigh number and $Ek$ is the Ekman number.

==> AAHG-macros.tex <==
\newcommand*{\Rr}{\mathbb{R}}
\providecommand*{\C}{}
\renewcommand*{\C}{\mathbb{C}}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Z}{\mathbb{Z}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\T}{\mathbb{T}}
\newcommand*{\A}{\mathbb{A}}
\newcommand*{\E}{\mathbb{E}}
\newcommand*{\K}{\mathbb{K}}
\newcommand*{\F}{\mathbb{F}}
\newcommand*{\D}{\mathbb{D}}
\newcommand*{\Ham}{\mathbb{H}}
\newcommand*{\hs}{\mathbb{H}}
\renewcommand*{\P}{\mathbb{P}}
\newcommand*{\e}{\mathrm{e}}
\newcommand*{\cc}{\mathrm{c}}
\newcommand*{\eps}{\varepsilon}
\newcommand*{\al}{\alpha}
\newcommand*{\Om}{\Omega}
\newcommand*{\bd}{\partial}
\newcommand*{\h}[1]{\hat{#1}}
\newcommand*{\s}[1]{\mathscr{#1}}
\newcommand*{\m}[1]{\mathcal{#1}}
\newcommand*{\fr}[1]{\mathfrak{#1}}
\newcommand*{\dn}{\mathrm{d}}
\newcommand*{\diff}{\mathrm{d}}
\newcommand*{\ds}{\,\mathrm{d}}
\renewcommand*{\d}{\;\mathrm{d}}
\newcommand*{\Der}{\mathrm{D}}
\newcommand*{\der}[2]{\frac{\dn #1}{\dn #2}}
\newcommand*{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand*{\abs}[1]{\left |#1 \right|}
\newcommand*{\abss}[1]{|#1|}
\newcommand*{\absb}[1]{\big|#1\big|}
\newcommand*{\norm}[1]{\left \|#1 \right\|}
\newcommand*{\norms}[1]{\|#1\|}
\newcommand*{\normb}[1]{\big\|#1 \big\|}
\newcommand*{\braket}[1]{\langle #1 \rangle}
\newcommand*{\Braket}[1]{\left\langle #1 \right\rangle}
\newcommand*{\op}[1]{\operatorname{#1}}
\newcommand*{\sgn}{\op{sgn}}
\newcommand*{\ti}[1]{\tilde{#1}}
\newcommand*{\ubar}[1]{\underline{#1}}
\newcommand*{\tbf}[1]{\textup{\textbf{#1}}}
\newcommand*{\trm}[1]{\textup{\textrm{#1}}}
\newcommand*{\id}[1]{\op{id}_{#1}}
\newcommand*{\anon}{\,\cdot\,}
\renewcommand*{\Re}{\op{Re}}
\renewcommand*{\Im}{\op{Im}}
\newcommand*{\Ker}{\op{ker}}
\newcommand*{\Image}{\op{im}}
\newcommand*{\Span}{\op{span}}
\newcommand*{\supp}{\op{supp}}
\newcommand*{\trans}[1]{\tensor*[^t]{#1}{}}
\newcommand*{\smooth}[1]{\m{C}_c^\infty(#1)}
\newcommand*{\arccot}{\op{arccot}}
\newcommand*{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand*{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand*{\noorm}[1]{\left|\left \|#1 \right\|\right|}
\newcommand*{\MLoc}{\m M_{c,\text{loc}}}
\newcommand*{\BM}{Brownian motion~}
\renewcommand*{\And}{\quad \text{and} \quad}
\newcommand*{\For}{\quad \text{for }}
\newcommand*{\ForAll}{\quad \text{for all }}
\newcommand*{\nab}{\nabla}
\newcommand*{\trdeg}{\op{tr\,deg}}
\newcommand*{\gr}{\op{gr}}
\newcommand*{\rees}{\op{Rees}}
\newcommand*{\Spec}{\op{Spec}}
\renewcommand*{\hom}[2]{\op{Hom}(#1, #2)}
\renewcommand*{\div}{\op{div}}
\newcommand*{\bbraket}[1]{\left \langle \! \left \langle #1 \right \rangle \! \right \rangle}
\newcommand*{\power}[1]{{#1}[\![X]\!]}
\newcommand*{\laurent}[1]{{#1}(\!(X)\!)}
\DeclareMathOperator*{\Dlim}{D-lim}
\DeclareMathOperator*{\Clim}{C-lim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\newcommand*{\mr}{\mathring}
\newcommand*{\smallO}{
  \mathchoice
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptscriptstyle\mathcal{O}$}}%
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%
  }

\newcommand{\sperp}{
{\mathchoice
{\mbox{\smaller$\bm\perp$}}
{\mbox{\smaller$\bm\perp$}}
{\mbox{\smaller[5]$\bm\perp$}}
{\mbox{\smaller[6]$\bm\perp$}}
}
}

\newcommand*{\iu}{\mathrm{i}}

\newcommand*{\smallbar}[1]{\overline{#1}}
\let\temp\bar
\let\bar\smallbar
\let\smallbar\temp
\let\temp\undefined

\newcommand*{\Hu}{\mathbb{H}}
\let\temp\H
\let\H\Hu
\let\Hu\temp
\let\temp\undefined

\newcommand*{\nsind}{\llbracket 2, N \rrbracket}

\newcommand*{\cub}{\fr{u}}
\newcommand*{\cubder}{\fr{m}}
\newcommand*{\dist}{\fr{d}}
\newcommand*{\Dist}{\fr{D}}
\newcommand*{\euc}{\fr{e}}
\newcommand*{\Euc}{\fr{E}}

\newcommand*{\out}[2]{{#1}_{#2}^{\textnormal{out}}}
\newcommand*{\inn}[2]{{#1}_{#2}^{\textnormal{in}}}
\newcommand*{\app}[2]{{#1}_{#2}^{\textnormal{app}}}
\newcommand*{\cut}[2]{{#1}_{#2}^{\textnormal{cut}}}
\newcommand*{\res}{{\textnormal{res}}}
\newcommand*{\match}{{\textnormal{m}}}
\newcommand*{\tb}{t_{\mathrm{b}}}
\newcommand*{\sft}{\mathsf{t}}
\newcommand*{\sfx}{\mathsf{x}}

\newcommand*{\Is}{{1}}
\newcommand*{\const}{\texttt{c}}
\newcommand*{\func}{\texttt{f}}
\newcommand*{\poly}{\mathsf{p}}

\newcommand*{\bigsub}[1]{{\mathclap{\substack{#1}}}\,}
\newcommand*{\Aop}{\m{A}}
\newcommand*{\Bop}{\m{B}}
\newcommand*{\Eta}{\mathsf{H}}
\newcommand*{\neweps}{\zeta}

\newcommand{\CG}[1]{{\color{green!60!black}\textbf{CG:} #1}}
\newcommand{\SC}[1]{{\color{red}\textbf{SC:} #1}}
\newcommand{\JA}[1]{{\color{blue} \textbf{JA:} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\green}[1]{{\color{green} #1}}

\newcommand*{\bR}{\mathbf{R}}
\newcommand*{\om}{\omega}
\newcommand*{\innind}{\s{I}}
\renewcommand*{\P}{\mathcal{P}}
\newcommand*{\inv}{{^{-1}}}
\newcommand*{\Ph}{\mathcal{P}}
\newcommand*{\Phs}{\Phi}
\newcommand*{\Phns}{\phi}
\newcommand*{\vbar}{\underline{v}}
\newcommand*{\half}{\frac 12}
\newcommand*{\ie}{i.\,e}
\newcommand*{\f}{\frac}
\DeclareMathOperator{\divr}{div}
\newcommand*{\fu}{\mathfrak{u}}
\newcommand*{\ft}{\mathfrak{t}}
\newcommand*{\fm}{\mathfrak{m}}
\newcommand*{\rd}{\partial}
\newcommand*{\fd}{\mathfrak{d}}
\renewcommand*{\D}{\mathcal{D}}
\newcommand*{\ls}{\lesssim}
\newcommand*{\gs}{\gtrsim}
\newcommand*{\calM}{\mathcal{M}}
\newcommand*{\calJ}{\mathcal{J}}
\newcommand*{\calB}{\mathcal{B}}
\newcommand*{\Php}{\bar{\Ph}}
\newcommand*{\Phsp}{\bar{\Phs}}
\newcommand*{\mup}{\bar{\mu}}
\newcommand*{\psip}{\bar{\psi}}
\newcommand*{\muT}{\hat{\mu}}
\newcommand*{\xiT}{\hat{\xi}}
\newcommand*{\xip}{\bar{\xi}}
\newcommand*{\bfd}{\mathbf{d}}
\newcommand*{\bfA}{\mathbf{A}}
\newcommand*{\bfr}{\mathbf{r}}
\newcommand*{\bfG}{\mathbf{G}}
\newcommand*{\PhT}{\hat{\Ph}}
\newcommand*{\PhsT}{\hat{\Phs}}
\newcommand*{\psiT}{\hat{\psi}}
\newcommand*{\AT}{\hat{A}}
\newcommand*{\rT}{\hat{r}}
\newcommand*{\lT}{\hat{l}}
\newcommand*{\XiT}{\hat{\Xi}}
\newcommand*{\calR}{\mathcal{R}}
\newcommand*{\calL}{\mathcal{L}}
\newcommand*{\calI}{\mathcal{I}}
\newcommand*{\calD}{\mathcal{D}}
\newcommand*{\calW}{\mathcal{W}}
\newcommand*{\taut}{\tilde{\tau}}
\newcommand*{\La}{\Lambda}
\newcommand*{\LaT}{\hat{\La}}
\newcommand*{\Lap}{\bar{\La}}
\newcommand*{\RT}{\hat{R}}
\newcommand*{\Rp}{\bar{R}}
\newcommand*{\PiT}{\hat{\Pi}}
\newcommand*{\Sigt}{\widetilde{\Sigma}}
\newcommand*{\Sigs}{\Sigma^*}
\newcommand*{\mus}{\mu^*}
\newcommand*{\calDt}{\widetilde{\calD}}
\newcommand*{\calDs}{\calD^*}
\newcommand*{\muts}{\tilde{\mu}^*}
\newcommand*{\Sigts}{\widetilde{\Sigma}^*}
\newcommand*{\calE}{\mathcal{E}}
\newcommand*{\ep}{\epsilon}
\newcommand*{\calQ}{\mathcal{Q}}
\newcommand*{\calN}{\mathcal{N}}
\newcommand*{\calG}{\mathcal{G}}
\newcommand*{\PG}{\calG}
\newcommand*{\PGT}{\hat{\PG}}
\newcommand*{\PGp}{\bar{\PG}}
\newcommand*{\calT}{\mathcal{T}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calS}{\mathcal{S}}
\DeclareMathOperator{\Lip}{Lip}
\newcommand*{\vb}{\vbar}
\newcommand*{\calV}{\mathcal{V}}


\newcommand{\AxisRotator}[1][rotate=0]{%
    \tikz [x=0.25cm,y=0.7cm,line width=.1ex,-stealth,#1] \draw (0,0) arc (-150:150:1 and 1);%
}

% \newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\note}[1]{{\color{blue}#1}}
% \newcommand{\anim}[1]{{\color{magenta}#1}}
% \newcommand{\resp}[1]{{\color{magenta}#1}}

\DeclareMathOperator*{\esssup}{ess\,sup}
\newcommand{\pol}{\Phi}
\newcommand{\tor}{\Theta}
\newcommand{\horg}{\nabla_{x,y}}
\newcommand{\hord}{\nabla_{x,y}^2}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\curl}{curl}


\newcommand{\Pp}{\mathbb{P}}
% \newcommand{\Rm}{\mathrm{Rm}}
% \newcommand{\R}{\mathrm{R}}
% \newcommand*{\Ra}{\mathrm{Ra}}
% \newcommand*{\Ro}{\mathrm{Ro}}
% \newcommand*{\Pe}{\mathrm{Pe}}
% \newcommand*{\Ek}{\mathrm{Ek}}
% \newcommand*{\Pm}{\mathrm{Pm}}
% \newcommand*{\Rmod}{\mathrm{Ra}^{*}}

\newcommand{\Rm}{ \mbox{\textit{Rm}} }
\newcommand{\R}{\mbox{\textit{R}}}
\newcommand{\Ra}{\mbox{\textit{Ra}}}
\newcommand{\Ro}{\mbox{\textit{Ro}}}
\newcommand{\Pe}{\mbox{\textit{Pe}}}
\newcommand{\Ek}{\mbox{\textit{Ek}}}
\newcommand{\Pm}{\mbox{\textit{Pm}}}
\newcommand{\Rmod}{\mbox{\textit{Ra}}}
